Automatic Cerebral Vessel Extraction in TOF-MRA Using Deep Learning

Deep learning approaches may help radiologists in the early diagnosis and timely treatment of cerebrovascular diseases. Accurate cerebral vessel segmentation of Time-of-Flight Magnetic Resonance Angiographs (TOF-MRAs) is an essential step in this process. This study investigates deep learning approaches for automatic, fast and accurate cerebrovascular segmentation for TOF-MRAs. The performance of several data augmentation and selection methods for training a 2D and 3D U-Net for vessel segmentation was investigated in five experiments: a) without augmentation, b) Gaussian blur, c) rotation and flipping, d) Gaussian blur, rotation and flipping and e) different input patch sizes. All experiments were performed by patch-training both a 2D and 3D U-Net and predicted on a test set of MRAs. Ground truth was manually defined using an interactive threshold and region growing method. The performance was evaluated using the Dice Similarity Coefficient (DSC), Modified Hausdorff Distance and Volumetric Similarity, between the predicted images and the interactively defined ground truth. The segmentation performance of all trained networks on the test set was found to be good, with DSC scores ranging from 0.72 to 0.83. Both the 2D and 3D U-Net had the best segmentation performance with Gaussian blur, rotation and flipping compared to other experiments without augmentation or only one of those augmentation techniques. Additionally, training on larger patches or slices gave optimal segmentation results. In conclusion, vessel segmentation can be optimally performed on TOF-MRAs using a trained 3D U-Net on larger patches, where data augmentation including Gaussian blur, rotation and flipping was performed on the training data.

==> Bibliography.tex <==
@article{Wermer2007,
  title={Risk of Rupture of Unruptured Intracranial Aneurysms in Relation to Patient and Aneurysm Characteristics},
  author={Wermer, M.J.H. and van der Schaaf, I.C. and Alagra A. and Rinkel, G.J.E.},
  journal={Stroke},
  volume={38},
  pages={1404-1410},
  year={2007}
}

@article{Wardlaw2000,
	title={The detection and management of unruptured intracranial aneurysms},
	author={Wardlaw, J.M. and White, P.M.},
	journal={Brain},
	volume={123},
	pages={205-221},
	year={2000}
}

@article{vanKammen2019,
	title={External Validation of the ELAPSS Score for Prediction of Unruptured Intracranial Aneurysm Growth Risk},
	author={van Kammen, M.S. and others},
	journal={Jornal of Stroke (JoS)},
	volume={21},
	number={3},
	pages={340-346},
	year={2019}
}

@article{Keedy2006,
	title={An overview of intracranial aneurysms},
	author={Keedy, A.},
	journal={McGill journal of medicine (MJM)},
	volume={9},
	number={2},
	pages={141-146},
	year={2006}
}

@article{Hentschke2012,
	title={Automatic Cerebral Aneurysm Detection in Multimodal Angiographic Images},
	author={Hentschke, C.M. and Beuing, O. and Nickl, R. and Tönnies, K.D.},
	journal={IEEE Nuclear Science Symposium Conference Record},
	pages={3116-3120},
	year={2011}
}

@article{Arimura2006,
	title={Computerized detection of intracranial aneurysms for three-dimensional MR angiography: Feature extraction of small protrusions based on a shape-based difference image technique},
	author={Arimura, H. and Li, Q. and Korogi, Y. and Hirai, T. and Katsuragawa, S. and Yamashita, Y. and Tsuchiya, K. and Doi, K.},
	journal={The American Association of Physicists in Medicine (AAPM)},
	volume={33},
	number={2},
	pages={394-401},
	year={2006}
}

@article{Lindgren2016,
	title={Irregular Shape of Intracranial Aneurysm Indicates Rupture Risk Irrespective of Size in a Population-Based Cohort},
	author={Lindgren, A.E. and Koivisto, T. and Björkman, J. and von und zu Fraunberg, M. and Helin, K. and Jääskeläinen, J.E. and Frösen, J.},
	journal={Stroke},
	volume={47},
	pages={1219-1226},
	year={2016}
}

@article{Raghavan2005,
	title={Quantified aneurysm shape and rupture risk},
	author={Raghavan, M.L. and Ma, B. and Harbaugh, R.E.},
	journal={Journal of Neurosurgery},
	volume={102},
	pages={355-362},
	year={2005}
}

@article{Gilhuijs1998,
	title={Computerized analysis of breast lesions in three dimensions using dynamic magnetic-resonance imaging},
	author={Gilhuijs, K.G.A. and Giger, M.L. and Bick, U.},
	journal={The American Association of Physicists in Medicine (AAPM)},
	volume={25},
	number={9},
	pages={1647-1654},
	year={1998}
}

@article{Hayashi2003,
	title={Feasibility of a Curvature-based Enhanced Display System for Detecting Cerebral Aneurysms in MR Angiography},
	author={Hayashi, N. and Masutani, Y. and Masumoto, T. and Mori, H. and Kunimatsu, A. and Abe, O. and Aoki, S. and Ohtomo, K. and Takano, N. and Matsumoto, K.},
	journal={Matnetic Resonance in Medical Sciences},
	volume={2},
	number={1},
	pages={29-36},
	year={2003}
}

@article{Chang2019,
	title={Improving the Otsu method for MRA image vessel extraction via resampling and ensemble learning},
	author={Chang, Y.},
	journal={Healthcare Technology Letters},
	volume={6},
	number={4},
	pages={115-120},
	year={2019}
}

@article{Fang2011,
	title={3D Model-based method for vessel segmentation in TOF-MRA},
	author={Fang, K. and Wang, D. and Lui, L.M. and Zhou, S. and Chu, W.C.W. and Ahuja, A.T. and Heng, P.A.},
	journal={Proceedings of the 2011 International Conference on Machine Learning and Cybernetics},
	volume={Grulin},
	pages={1607-1611},
	year={2011}
}

@article{Lu2016,
	title={A vessel segmentation method for multi-modality angiographic images based on multi-scale filtering and statistical models},
	author={Lu, P. and Xia, J. and Li, Z. and Xiong, J. and Yang, J. and Zhou, S. and Wang, L. and Chen, M. and Wang, C.},
	journal={Biomedical Engineering OnLine},
	volume={15},
	number={120},
	year={2016}
}

@article{Livne2019,
	title={A U-Net Deep Learning Framework for High Performance Vessel Segmentation in Patients With Cerebrovascular Disease},
	author={Livne, M. and Rieger, J. and Aydin, O.U. and Taha, A.A. and Akay, E.M. and Kossen, T. and Sobesky, J. and Kelleher, J.D. and Hildebrand, K. and Frey, D. and Madai, V.I.},
	journal={Frontiers in Neuroscience},
	volume={13},
	number={97},
	year={2019}
}

@article{Ronneberger2015,
	title={U-net: Convolutional networks for biomedical image segmentation},
	author={Ronneberger, O. and Fischer, P. and Brox, T.},
	journal={Medical Image Computing and Computer-Assisted Intervention (MICCAI)},
	volume={9351},
	pages={234-241},
	year={2015}
}

@article{Frangi1998,
	title={Multiscale Vessel Enhancement Filtering},
	author={Frangi, A.F. and Niessen, W.J. and Vincken K.L. and Viergever, M.A.},
	journal={Lecture Notes in Computer Science},
	volume={1496},
	pages={130-137},
	year={1998}
}

@article{Gan2005,
	title={Statistical cerebrovascular segmentation in three-dimensional rotational angiography based on maximum intensity projections},
	author={Gan, R. and Wong, W.C.K and Chung, A.C.S.},
	journal={Medical Physics},
	volume={32},
	number={9},
	pages={3017-3028},
	year={2005}
}

@article{Phellan2007,
	title={Vascular Segmentation in TOF MRA Images of the Brain Using a Deep Convolutional Neural Network},
	author={Phellan, R. and Peixinho, A. and Falcão, A. and Forkert, N.D.},
	journal={Lecture Notes in Computer Science},
	volume={10552},
	pages={39-46},
	year={2017}
}

@article{McInerney1997,
	title={Medical Image Segmentation Using Topologically Adaptable Surface},
	author={McInerney, T. and Terzopoulos, D.},
	journal={Lecture Notes in Computer Science},
	volume={1205},
	pages={23-32},
	year={1997}
}

@article{Chen2003,
	title={Gibbs Prior Models, Marching Cubes, and Deformable Models: A Hybrid Framework for 3D Medical Image Segmentation},
	author={Chen, T. and Metaxas, D.},
	journal={Lecture Notes in Computer Science},
	volume={2879},
	pages={703-710},
	year={2003}
}

@article{Katan2018,
	title={Global Burden of Stroke},
	author={Katan, M. and Luft, A.},
	journal={Seminars in Neurology},
	volume={38},
	number={2},
	pages={208-211},
	year={2018}
}

@article{Tustison2010-B-Spline,
	title={N4ITK: Improved N3 Bias Correction With Robust B-Spline Approximation},
	author={Tustison, N.J. and Avants, B.B. and Cook, P.A. and Gee, J.C.},
	journal={IEEE transactions on medical imaging},
	pages={708-711},
	year={2010}
}

@article{Tustison2010,
	title={N4ITK: Improved N3 Bias Correction},
	author={Tustison, N.J. and Avants, B.B. and Cook, P.A. and Zheng, Y. and Egan, A. and Yushkevich, P.A. and Gee, J.C.},
	journal={IEEE Transactions on Medical Imaging},
	volume={29},
	number={6},
	pages={1310-1320},
	year={2010}
}

@article{Robitaille2012,
	title={Tissue-based MRI intensity standardization: application to multicentric datasets},
	author={Robitaille, N. and Mouiha, A. and Crépeault, B. and Valdivia, F. and Duchesne, S. and {The Alzheimer's Disease Neuroimaging Initiative}},
	journal={International journal of biomedical imaging},
	year={2012}
}

@article{Ellingson2012,
	title={Comparison between intensity normalization techniques for dynamic susceptibility contrast (DSC)-MRI estimates of cerebral blood volume (CBV) in human gliomas},
	author={Ellingson, B.M. and Zaw, T. and Cloughesy, T.F. and Naeini, K.M. and Lalezari, S. and Mong, S. and Lai, A. and Nghiemphu, P.L. and Pope, W.B.},
	journal={Journal of magnetic reesonance imaging (JMRI)},
	volume={35},
	number={6},
	pages={1472-1477},
	year={2012}
}

@article{Song2017,
	title={A Review of Methods for Bias Correction in Medical Images},
	author={Song, S. and Zheng, Y. and He, Y.},
	journal={Biomedical Engineering Review},
	volume={1},
	number={1},
	year={2017}
}

@book{Toennies-regiongrowing,
	author    = {Toennies, K.D.}, 
	title     = {Guide to Medical Image Analysis - Advances in Computer Vision and Pattern Recognition},
	publisher = {Springer},
	year      = 2012,
	note      = {pp. 199-200},
	isbn      = {978-1-4471-2750-5}
}

@article{Greving2013,
	title={Development of the PHASES score for prediction of risk of rupture of intracranial aneurysms: a pooled analysis of six prospective cohort studies},
	author={Greving, J.P. and Wermer, M.J.H. and Brown Jr, R.D. and Morita, A. and Juvela, S. and Yonekura, M. and Ishibashi, T. and Torner, J.C. and Nakayama, T. and Rinkel, G.J.E. and Algra, A.},
	journal={The Lancet Neurology},
	volume={13},
	pages={59-66},
	year={2014}
}

@article{Yang2011,
	title={Computer-Aided Detection of Intracranial Aneurysms in MR Angiography},
	author={Yang, X. and Blezek, D.J. and Cheng, L.T.E. and Ryan, W.J. and Kallmes, D.F. and Erickson, B.J.},
	journal={Journal of Digital Imaging},
	volume={24},
	number={1},
	pages={86-95},
	year={2011}
}

@article{Duan2019,
	title={Automatic detection on intracranial aneurysm from digital subtraction angiography with cascade convolutional neural networks},
	author={Duan, H. and Huang, Y. and Liu, L. and Dai, H. and Chen, L. and Zhou, L.},
	journal={BioMedical Engineering OnLine},
	volume={18},
	number={1},
	year={2019}
}

@book{Toennies-dsc,
	author    = {Toennies, K.D.}, 
	title     = {Guide to Medical Image Analysis - Advances in Computer Vision and Pattern Recognition},
	publisher = {Springer},
	year      = 2012,
	note      = {pp. 418},
	isbn      = {978-1-4471-2750-5}
}

@article{Taha2015,
	title={Metrics for evaluating 3D medical image segmentation: analysis, selection, and tool},
	author={Taha, A.A. and Hanbury, A.},
	journal={BMC Medical Imaging},
	volume={15},
	number={29},
	year={2015}
}

@book{Toennies-sensitivity,
	author    = {Toennies, K.D.}, 
	title     = {Guide to Medical Image Analysis - Advances in Computer Vision and Pattern Recognition},
	publisher = {Springer},
	year      = 2012,
	note      = {pp. 420-421},
	isbn      = {978-1-4471-2750-5}
}

@article{Lorensen1987,
	title={Marching cubes: A high resolution 3D surface construction algorithm},
	author={Lorensen, W.E. and Cline, H.E.},
	journal={ACM SIGGRAPH Computer Graphics},
	volume={21},
	number={4},
	year={1987}
}

@article{Koenderink1992,
	title={Surface shape and curvature scales},
	author={Koenderink, J.J. and van Doorn, A.J.},
	journal={Image and Vision Computing},
	volume={10},
	number={8},
	pages={557-564},
	year={1992}
}

@article{Chen2017,
	title={3D intracranial artery segmentation using a convolutional autoencoder},
	author={Chen, L. and Xie, Y. and Sun, J. and Balu, N. and Mossa-Basha, M. and Pimentel, K. and Hatsukami, T.S. and Hwang, J. and Yuan, C.},
	journal={IEEE International Conference on Bioinformatics and Biomedicine (BIBM)},
	pages={704-707},
	year={2017}
}

@article{Lawonn2019,
	title={A Geometric Optimization Approach for the Detection and Segmentation of Multiple Aneurysms},
	author={Lawonn, K. and Meuschke, M. and Wickenhöfer, R. and Preim, B. and Hildebrandt, K.},
	journal={Eurographics Conference on Visualization (EuroVis)},
	volume={38},
	number={3},
	year={2019}
}

@misc{Adam,
	title = {Aneurysm Detection And segMentation (ADAM) Challenge},
	howpublished = {\url{http://adam.isi.uu.nl}},
	note = {Accessed: 2020-10-20}
}

@misc{ANTs,
	title = {Advanced Normalization Tools (ANTs)},
	howpublished = {\url{http://stnava.github.io/ANTs/}},
	note = {Accessed: 2020-10-23}
}

@article{Chicco2020,
	title={The advantages of the Matthews correlation coefficient (MCC) over F1 score and accuracy in binary classification evaluation},
	author={Chicco, D. and Jurman, G.},
	journal={BMC Genomics},
	volume={21},
	number={6},
	year={2020}
}

@article{Kim2015,
	title={T test as a parametric statistic},
	author={Kim, T.K.},
	journal={Korean Journal of Anesthesiology},
	volume={68},
	number={6},
	pages={540-546},
	year={2015}
}

@article{Shorten2019,
	title={A survey on Image Data Augmentation for Deep Learning},
	author={Shorten, C. and Khoshgoftaar, T.M.},
	journal={Journal of Big Data},
	volume={6},
	number={60},
	year={2019}
}

@article{Hentschke2012_newfeature,
	title={A new feature for automatic aneurysm detection},
	author={Hentschke, C.M. and Tönnies, K.D. and Beuing, O. and Nickl, R.},
	journal={9th IEEE International Symposium on Biomedical Imaging (ISBI)},
	pages={800-803},
	year={2012}
}

@article{Wiebers2003,
	title={Unruptured intracranial aneurysms: natural history, clinical outcome, and risks of surgical and endovascular treatment},
	author={Wiebers, D.O. and others},
	journal={Lancet},
	volume={362},
	pages={102-110},
	year={2003}
}

@article{Whitley2002,
	title={Statistics review 6: Nonparametric methods},
	author={Whitley, E. and Ball, J.},
	journal={Critical Care},
	volume={6},
	number={6},
	pages={509-513},
	year={2002}
}

@article{Ritter2011,
	title={Medical Image Analysis},
	author={Ritter, F. and others},
	journal={IEEE Pulse},
	volume={2},
	number={6},
	pages={60-70},
	year={2011}
}
